Enhancement of a state-of-the-art RL-based detection algorithm for Massive MIMO radars

In the present work, a reinforcement learning (RL) based adaptive algorithm to optimise the transmit beampattern for a colocated massive MIMO radar is presented. Under the massive MIMO regime, a robust Wald type detector, able to guarantee certain detection performances under a wide range of practical disturbance models, has been recently proposed. Furthermore, an RL/cognitive methodology has been exploited to improve the detection performance by learning and interacting with the surrounding unknown environment. Building upon previous findings, we develop here a fully adaptive and data driven scheme for the selection of the hyper-parameters involved in the RL algorithm. Such an adaptive selection makes the Wald RL based detector independent of any ad hoc, and potentially suboptimal, manual tuning of the hyper-parameters. Simulation results show the effectiveness of the proposed scheme in harsh scenarios with strong clutter and low SNR values.

==> figures/AlgorithmComparison/PerformanceComparison/Scenario5/alpha_Scenario5.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.761\textwidth,
height=0.32\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=200,
xlabel style={font=\color{white!15!black}},
xlabel={Discrete time $k$},
ymin=0.2,
ymax=0.6,
ylabel style={font=\color{white!15!black}},
ylabel={$\alpha_k$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.599999999999996\\
2	0.598039258448798\\
3	0.596071053906841\\
4	0.594088227621995\\
5	0.59208420701342\\
6	0.590053245199381\\
7	0.587990602159822\\
8	0.585892657132865\\
9	0.583756948154839\\
10	0.58158214098129\\
11	0.579367935277034\\
12	0.577114920372464\\
13	0.574824395684704\\
14	0.572498171961363\\
15	0.570138368916587\\
16	0.567747222882773\\
17	0.565326915218143\\
18	0.562879428870489\\
19	0.560406437163674\\
20	0.557909225927842\\
21	0.5553886477932\\
22	0.552845105922431\\
23	0.55027856364159\\
24	0.547688576206105\\
25	0.545074341101903\\
26	0.542434763607375\\
27	0.539768534633058\\
28	0.537074217978982\\
29	0.534350344053976\\
30	0.531595506820921\\
31	0.52880846036968\\
32	0.52598821121786\\
33	0.523134102345441\\
34	0.520245885198245\\
35	0.517323776503877\\
36	0.514368497714709\\
37	0.511381296134505\\
38	0.508363948148632\\
39	0.505318746281017\\
40	0.502248472863471\\
41	0.499156363777676\\
42	0.496046065928232\\
43	0.492921591810947\\
44	0.489787273811678\\
45	0.486647719826672\\
46	0.48350777059528\\
47	0.480372457954062\\
48	0.477246962220856\\
49	0.47413656622984\\
50	0.471046603250998\\
51	0.467982396177543\\
52	0.464949185943607\\
53	0.461952048093135\\
54	0.458995797679622\\
55	0.456084884132809\\
56	0.45322327926443\\
57	0.450414363070814\\
58	0.44766081328868\\
59	0.444964505632397\\
60	0.442326432152715\\
61	0.439746645091322\\
62	0.437224232877382\\
63	0.434757333483881\\
64	0.432343188259238\\
65	0.429978236673756\\
66	0.427658249349694\\
67	0.425378493528289\\
68	0.423133922070871\\
69	0.420919374523759\\
70	0.418729777016402\\
71	0.416560327076595\\
72	0.414406650013147\\
73	0.412264915391358\\
74	0.410131905226235\\
75	0.408005029616073\\
76	0.405882290280892\\
77	0.403762197408146\\
78	0.40164364984539\\
79	0.399525792526285\\
80	0.397407867644427\\
81	0.395289077183387\\
82	0.393168473805109\\
83	0.391044894797623\\
84	0.388916949964653\\
85	0.386783069338725\\
86	0.384641610873559\\
87	0.382491022357976\\
88	0.380330046256172\\
89	0.378157951555354\\
90	0.375974773450875\\
91	0.373781540158529\\
92	0.371580466494703\\
93	0.369375096111846\\
94	0.367170378240246\\
95	0.364972670117074\\
96	0.362789662486326\\
97	0.360630232036747\\
98	0.358504230777382\\
99	0.356422227527569\\
100	0.354395220411201\\
101	0.35243434114207\\
102	0.350550571818434\\
103	0.348754492984477\\
104	0.347056078153741\\
105	0.345464545292169\\
106	0.343988270506252\\
107	0.34263476398428\\
108	0.341410703645519\\
109	0.340322018371726\\
110	0.339374010338118\\
111	0.338571504815857\\
112	0.337919015673165\\
113	0.337420915304002\\
114	0.337081598461292\\
115	0.336905630126623\\
116	0.336897867934715\\
117	0.337063549846786\\
118	0.337408338037713\\
119	0.337938310823258\\
120	0.338659896460831\\
121	0.339579746238499\\
122	0.340704549516505\\
123	0.342040799893336\\
124	0.343594528445269\\
125	0.345371025546473\\
126	0.347374575389854\\
127	0.349608225457543\\
128	0.352073605996677\\
129	0.354770802381573\\
130	0.357698267886866\\
131	0.360852749052864\\
132	0.364229184596736\\
133	0.367820535831566\\
134	0.371617514807972\\
135	0.375608196686036\\
136	0.379777533027091\\
137	0.384106817588432\\
138	0.388573188350624\\
139	0.393149270682674\\
140	0.397803069768424\\
141	0.402498201942854\\
142	0.407194515395795\\
143	0.411849096888598\\
144	0.416417602983363\\
145	0.420855804071025\\
146	0.425121198393645\\
147	0.429174548272013\\
148	0.432981212398016\\
149	0.43651218987792\\
150	0.439744841936664\\
151	0.442663302288185\\
152	0.445258616347478\\
153	0.447528658404111\\
154	0.449477868198405\\
155	0.451116833704534\\
156	0.45246173637543\\
157	0.453533675443898\\
158	0.454357897788234\\
159	0.454962970108243\\
160	0.455379928326989\\
161	0.455641417297783\\
162	0.45578079530168\\
163	0.455831138896086\\
164	0.455824069229515\\
165	0.455788353564472\\
166	0.455748323279572\\
167	0.455722275846128\\
168	0.455721151757264\\
169	0.455747841366257\\
170	0.455797429893803\\
171	0.455858512728741\\
172	0.45591544231476\\
173	0.455951091386519\\
174	0.45594955092811\\
175	0.455898220870889\\
176	0.455789025634251\\
177	0.455618921585656\\
178	0.455390267579753\\
179	0.45511173486812\\
180	0.454800037693658\\
181	0.45448194108238\\
182	0.454195161265931\\
183	0.453986444760453\\
184	0.453905639407823\\
185	0.453995897932536\\
186	0.454282049939228\\
187	0.454761360684113\\
188	0.455402071738774\\
189	0.456156151056617\\
190	0.45698638332614\\
191	0.457891446631354\\
192	0.458904197892123\\
193	0.460043206352517\\
194	0.461262778630237\\
195	0.462427475842214\\
196	0.463383498312239\\
197	0.464180614976823\\
198	0.464992964491696\\
199	0.465537472244557\\
200	0.465774481144152\\
};
\end{axis}
\end{tikzpicture}%

==> figures/AlgorithmComparison/PerformanceComparison/Scenario5/epsilon_Scenario5.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.761\textwidth,
height=0.32\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=200,
xlabel style={font=\color{white!15!black}},
xlabel={Discrete time $k$},
ymin=0.1,
ymax=0.8,
ylabel style={font=\color{white!15!black}},
ylabel={$\varepsilon_k$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.799999999999971\\
2	0.795096260221938\\
3	0.790178204250087\\
4	0.785232201433218\\
5	0.780245938851134\\
6	0.775208952339672\\
7	0.770113018924294\\
8	0.764952387138751\\
9	0.759723837412039\\
10	0.754426580334881\\
11	0.74906201438999\\
12	0.743633375213478\\
13	0.738145314727983\\
14	0.732603450233855\\
15	0.727013921041654\\
16	0.721382984259927\\
17	0.715716673046606\\
18	0.710020531276054\\
19	0.704299429414156\\
20	0.698557458473299\\
21	0.692797892957929\\
22	0.687023210052533\\
23	0.681235150920489\\
24	0.675434810539325\\
25	0.669622744452141\\
26	0.663799083531515\\
27	0.657963650718623\\
28	0.652116076219022\\
29	0.646255909484024\\
30	0.640382727353887\\
31	0.634496238035489\\
32	0.628596380315246\\
33	0.622683416822\\
34	0.61675801951598\\
35	0.610821345103121\\
36	0.604875097890798\\
37	0.598921577748948\\
38	0.592963711272987\\
39	0.587005064859118\\
40	0.58104983907518\\
41	0.57510284433189\\
42	0.569169458361092\\
43	0.563255566371464\\
44	0.557367485008003\\
45	0.55151187145037\\
46	0.545695619216324\\
47	0.539925742544017\\
48	0.534209251633077\\
49	0.528553021512168\\
50	0.522963657818215\\
51	0.517447363246435\\
52	0.512009808784093\\
53	0.506656014012125\\
54	0.501390240712271\\
55	0.496215903749172\\
56	0.491135502730598\\
57	0.486150577324497\\
58	0.481261688371796\\
59	0.476468426111793\\
60	0.47176944594853\\
61	0.467162531230639\\
62	0.462644681482812\\
63	0.45821222340708\\
64	0.453860940777446\\
65	0.449586218125209\\
66	0.445383191936563\\
67	0.441246902078352\\
68	0.437172435479018\\
69	0.43315505387352\\
70	0.429190297809441\\
71	0.425274060197554\\
72	0.421402624495729\\
73	0.417572665076736\\
74	0.41378121029374\\
75	0.410025571984628\\
76	0.406303248348253\\
77	0.402611809952578\\
78	0.398948780776191\\
79	0.395311527370094\\
80	0.391697169271987\\
81	0.388102522639593\\
82	0.384524086748018\\
83	0.38095807969726\\
84	0.377400525682264\\
85	0.373847391845516\\
86	0.370294768450564\\
87	0.366739082265595\\
88	0.363177329963793\\
89	0.359607316288384\\
90	0.356027880853456\\
91	0.352439097808574\\
92	0.348842434133396\\
93	0.345240854902843\\
94	0.341638867254388\\
95	0.338042498724971\\
96	0.334459209805631\\
97	0.330897744682397\\
98	0.327367927905409\\
99	0.323880417906125\\
100	0.32044643067134\\
101	0.31707744835637\\
102	0.313784928125969\\
103	0.310580026071273\\
104	0.307473349751913\\
105	0.304474750894273\\
106	0.301593167213654\\
107	0.298836519406391\\
108	0.296211666256606\\
109	0.293724417674888\\
110	0.291379602451846\\
111	0.289181184651658\\
112	0.287132419947649\\
113	0.285236040867444\\
114	0.283494457945821\\
115	0.28190996230694\\
116	0.280484914412044\\
117	0.279221903880973\\
118	0.278123866728104\\
119	0.277194149314201\\
120	0.276436512935954\\
121	0.275855079130369\\
122	0.275454222979609\\
123	0.275238429078151\\
124	0.275212131130548\\
125	0.275379559965201\\
126	0.275744624760115\\
127	0.276310847618953\\
128	0.277081362242243\\
129	0.278058974259341\\
130	0.279246265801376\\
131	0.280645712862742\\
132	0.282259773959669\\
133	0.284090905220117\\
134	0.286141461978583\\
135	0.288413460344667\\
136	0.290908192525476\\
137	0.293625713880963\\
138	0.296564243792068\\
139	0.299719542229186\\
140	0.303084335821584\\
141	0.306647868927883\\
142	0.310395646101319\\
143	0.314309413684019\\
144	0.318367402918927\\
145	0.322544828861853\\
146	0.326814612705949\\
147	0.331148273500694\\
148	0.33551692095352\\
149	0.339892274698997\\
150	0.344247636323225\\
151	0.348558747016763\\
152	0.352804474655337\\
153	0.356967288866557\\
154	0.361033501481027\\
155	0.364993272688258\\
156	0.368840408400644\\
157	0.372571996906089\\
158	0.376187945248557\\
159	0.379690470153355\\
160	0.383083571325812\\
161	0.386372472176826\\
162	0.389562970737859\\
163	0.392660625037653\\
164	0.395669723568492\\
165	0.398592069557101\\
166	0.40142572169252\\
167	0.404163945702966\\
168	0.406794692703276\\
169	0.409300893721229\\
170	0.411661736540755\\
171	0.413854898536861\\
172	0.415859500813489\\
173	0.417659379528923\\
174	0.419246172995031\\
175	0.42062170506801\\
176	0.421799206067133\\
177	0.422803062788506\\
178	0.423667035354389\\
179	0.424431181886486\\
180	0.42513800334698\\
181	0.425828487305245\\
182	0.426538772213185\\
183	0.427298062447688\\
184	0.428128117597618\\
185	0.429044081625418\\
186	0.430055801386183\\
187	0.43116833064583\\
188	0.432380592493015\\
189	0.433684503632412\\
190	0.435069073828308\\
191	0.436526051011427\\
192	0.438048010259443\\
193	0.43959783675547\\
194	0.441085042058411\\
195	0.442363132190634\\
196	0.443306368313799\\
197	0.443922412880202\\
198	0.44433743877198\\
199	0.444383683318968\\
200	0.444120935557187\\
};
\end{axis}
\end{tikzpicture}%

==> figures/AlgorithmDescription/alpha_parameter/AlphaParam_Target1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=0.761\textwidth,
height=0.5\textwidth,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={Discrete time $k$},
ymin=0.5,
ymax=0.9,
ylabel style={font=\color{white!15!black}},
ylabel={$P_D$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(0.55\textwidth,0.6 \textwidth)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0753187197439853\\
2	0.119780880153038\\
3	0.162505392485333\\
4	0.203526309669188\\
5	0.242876948507607\\
6	0.280587853036833\\
7	0.316685734192378\\
8	0.351192837937054\\
9	0.384126325587658\\
10	0.41549750058779\\
11	0.445310526023074\\
12	0.47356102208384\\
13	0.50023457897721\\
14	0.525305027687294\\
15	0.548732764323509\\
16	0.570462881149969\\
17	0.59042401479656\\
18	0.608532801889113\\
19	0.624735066833984\\
20	0.639224028160488\\
21	0.653020986012825\\
22	0.667245564916536\\
23	0.680895806268581\\
24	0.69390022246429\\
25	0.706186199729351\\
26	0.71769488579077\\
27	0.728386732509812\\
28	0.738247713334665\\
29	0.747285627186758\\
30	0.755536722578803\\
31	0.763058942129602\\
32	0.769924293286057\\
33	0.776208713866386\\
34	0.781976348617983\\
35	0.787282165649841\\
36	0.79217685272679\\
37	0.796714413816536\\
38	0.800944905344375\\
39	0.804912717384939\\
40	0.808659043909835\\
41	0.812223937899456\\
42	0.815642147082171\\
43	0.818935515139877\\
44	0.822112421096089\\
45	0.82517483933593\\
46	0.828118912238141\\
47	0.830942107336893\\
48	0.833639522547509\\
49	0.836202700792942\\
50	0.838624941449627\\
51	0.840902610886303\\
52	0.843041160307647\\
53	0.845053457788504\\
54	0.846956937381174\\
55	0.848766693217948\\
56	0.850491207266644\\
57	0.852129886153675\\
58	0.853670530723932\\
59	0.855095656039506\\
60	0.856392464882392\\
61	0.857557941582937\\
62	0.858592515743057\\
63	0.859502408886451\\
64	0.860309774526421\\
65	0.861047403210275\\
66	0.861747876518269\\
67	0.86243831980618\\
68	0.863141582075308\\
69	0.863873840760355\\
70	0.864633693049685\\
71	0.86539644455673\\
72	0.866130964623968\\
73	0.866816992806786\\
74	0.867449274089179\\
75	0.868030551576806\\
76	0.8685676030631\\
77	0.869073340731934\\
78	0.869556836046735\\
79	0.870019296960884\\
80	0.870456674166974\\
81	0.870805427620811\\
82	0.871143851889697\\
83	0.871496786376585\\
84	0.871863504566553\\
85	0.872238726047617\\
86	0.872618006135153\\
87	0.872998287736654\\
88	0.873377750686068\\
89	0.87375570808558\\
90	0.874132199102243\\
91	0.874507523674333\\
92	0.874882129293911\\
93	0.875256602422458\\
94	0.8756317067318\\
95	0.87600830654341\\
96	0.876387350265496\\
97	0.876769941981447\\
98	0.877157279321165\\
99	0.877550506450147\\
100	0.877950730931122\\
};
\addlegendentry{$\alpha$ = 0.20}

\addplot [color=blue, solid, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0321926675894971\\
2	0.0983862835654563\\
3	0.161652576444611\\
4	0.222009168112347\\
5	0.279475034941756\\
6	0.334070544472531\\
7	0.385817422603129\\
8	0.434738458246153\\
9	0.480856804367101\\
10	0.524195111973869\\
11	0.564774433505303\\
12	0.602612471166889\\
13	0.637721246645376\\
14	0.670103634475453\\
15	0.699747845205788\\
16	0.726618806664805\\
17	0.750643343521225\\
18	0.771685489271771\\
19	0.789516774692272\\
20	0.803879400592411\\
21	0.815022774997215\\
22	0.824030968949309\\
23	0.83136499556222\\
24	0.837318051424481\\
25	0.842149469149427\\
26	0.846075394739904\\
27	0.849267898824457\\
28	0.851863301274961\\
29	0.853973205884191\\
30	0.855692167494693\\
31	0.857100400715475\\
32	0.858264238559806\\
33	0.859235370852492\\
34	0.860059064496014\\
35	0.860773017509407\\
36	0.861404008887437\\
37	0.861961405981858\\
38	0.862450002372213\\
39	0.862867830058021\\
40	0.86321128990135\\
41	0.863479789172177\\
42	0.86368113038993\\
43	0.863827109579082\\
44	0.863932351452607\\
45	0.864011933888313\\
46	0.864079621135408\\
47	0.864138994555584\\
48	0.864186607686719\\
49	0.864227242778316\\
50	0.864269825350729\\
51	0.864317155909834\\
52	0.864378949789202\\
53	0.864463245455048\\
54	0.864564337561492\\
55	0.864674386213185\\
56	0.864790070198801\\
57	0.864906051317633\\
58	0.86501736590026\\
59	0.865124362665692\\
60	0.865221856721592\\
61	0.865298226652565\\
62	0.865347788407871\\
63	0.8653620666642\\
64	0.865330674345312\\
65	0.865241954364859\\
66	0.865088731294419\\
67	0.864877090313889\\
68	0.864624311463659\\
69	0.864348933932144\\
70	0.864071990024149\\
71	0.863814914474458\\
72	0.863595730194079\\
73	0.863421970797853\\
74	0.863290245309199\\
75	0.863198745808597\\
76	0.863146877342633\\
77	0.863133927791343\\
78	0.863165462017683\\
79	0.863255002323191\\
80	0.863416515968937\\
81	0.863749957078512\\
82	0.864068469091123\\
83	0.864313446801707\\
84	0.864489632391883\\
85	0.864610247268472\\
86	0.86468519005261\\
87	0.864720900394127\\
88	0.864721495260406\\
89	0.864689452309703\\
90	0.864625960624994\\
91	0.864531358319118\\
92	0.864405303634417\\
93	0.864246847834439\\
94	0.864054558566373\\
95	0.863826770921969\\
96	0.863561551036459\\
97	0.863256758152939\\
98	0.862910097219831\\
99	0.862519356631203\\
100	0.862082636509965\\
};
\addlegendentry{$\alpha$ = 0.50}

\addplot [color=black, solid, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0526001386730171\\
2	0.120459336879897\\
3	0.184988637330212\\
4	0.246223034213649\\
5	0.304200571869074\\
6	0.358961035788655\\
7	0.410544639321125\\
8	0.458991021425445\\
9	0.504338037679035\\
10	0.54662031481397\\
11	0.585867404157669\\
12	0.622101051888083\\
13	0.655331291219507\\
14	0.685550857791393\\
15	0.712727248886926\\
16	0.736789946011496\\
17	0.757610095331154\\
18	0.774969294032604\\
19	0.788535628429497\\
20	0.798029064258257\\
21	0.804182118250528\\
22	0.809427254519895\\
23	0.813520139988605\\
24	0.816734186322048\\
25	0.819284800026384\\
26	0.821342522867181\\
27	0.823030965053659\\
28	0.824439579203489\\
29	0.825627606749298\\
30	0.826634553015356\\
31	0.827484344482685\\
32	0.828191025447328\\
33	0.8287660361814\\
34	0.829223634078902\\
35	0.829586348423494\\
36	0.829872748615058\\
37	0.830090467243933\\
38	0.830244598676421\\
39	0.83034740783388\\
40	0.830414180852853\\
41	0.830468787413316\\
42	0.83052626706256\\
43	0.830585918973664\\
44	0.830642200983987\\
45	0.830694884341352\\
46	0.83074298472553\\
47	0.830788853457321\\
48	0.830841772570553\\
49	0.830914491485091\\
50	0.831014980619269\\
51	0.831142341066595\\
52	0.83129449457463\\
53	0.831466544756743\\
54	0.83164908893882\\
55	0.831841363683878\\
56	0.832049765832576\\
57	0.832282504731063\\
58	0.832540461623523\\
59	0.832826793607671\\
60	0.833147992077374\\
61	0.83349944008069\\
62	0.833873901108171\\
63	0.834260724889957\\
64	0.834651531075176\\
65	0.835040188666197\\
66	0.835425988238509\\
67	0.835809563839161\\
68	0.836190463968851\\
69	0.836553868619315\\
70	0.836875243508726\\
71	0.837129045556162\\
72	0.837298702952574\\
73	0.837374872229395\\
74	0.837360500165087\\
75	0.837270219497305\\
76	0.837121982197473\\
77	0.836935023316848\\
78	0.836726667028623\\
79	0.83651447935833\\
80	0.836310080984035\\
81	0.836195478765959\\
82	0.836160837994035\\
83	0.836181697570473\\
84	0.836238868688216\\
85	0.836323663842358\\
86	0.836433052879905\\
87	0.836566737843868\\
88	0.836725783159652\\
89	0.836911639046161\\
90	0.837125606173646\\
91	0.837368648596847\\
92	0.837641501738624\\
93	0.837944707837851\\
94	0.83827872641853\\
95	0.838643947354135\\
96	0.839040509598997\\
97	0.839468359534215\\
98	0.839927298628362\\
99	0.840417000982317\\
100	0.840937021112357\\
};
\addlegendentry{$\alpha$ = 0.80}

\end{axis}
\end{tikzpicture}%

==> figures/AlgorithmDescription/policy_improvement/EpsilonGreedy_Target1.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[%
width=75mm,
height=44mm,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=150,
xlabel style={font=\color{white!15!black}},
xlabel={Discrete time $k$},
ymin=0,
ymax=1,
ylabel style={font=\color{white!15!black}},
ylabel={$P_D$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
legend style={at={(27mm,2mm)}, anchor=south west, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0398443724408018\\
2	0.222654217594632\\
3	0.362483489018651\\
4	0.460154987906088\\
5	0.509923722564055\\
6	0.545475115373239\\
7	0.571129613524821\\
8	0.590911703445885\\
9	0.606849135829465\\
10	0.61848288479356\\
11	0.626555141179401\\
12	0.634860662962573\\
13	0.643013718160841\\
14	0.64773012033573\\
15	0.649008898949924\\
16	0.649386993830966\\
17	0.651006108240067\\
18	0.655022407394229\\
19	0.659313686613868\\
20	0.66248732338146\\
21	0.665061841877\\
22	0.665359646743906\\
23	0.665942015568197\\
24	0.668250027199666\\
25	0.668678257668906\\
26	0.668504531797288\\
27	0.668983289492891\\
28	0.669611950023586\\
29	0.669768396861156\\
30	0.666897848899048\\
31	0.664723048173474\\
32	0.666175864134105\\
33	0.668367195002266\\
34	0.668849773489478\\
35	0.667053929808853\\
36	0.667269528378142\\
37	0.671096864096758\\
38	0.675801208304931\\
39	0.678696078551709\\
40	0.678676670728341\\
41	0.678041558272706\\
42	0.67721460128183\\
43	0.677265260919424\\
44	0.67947726742183\\
45	0.682704182629138\\
46	0.686302480390254\\
47	0.688133381904481\\
48	0.687745804904938\\
49	0.687083238197666\\
50	0.686529405926262\\
51	0.685891295123721\\
52	0.685951707403234\\
53	0.686549969512016\\
54	0.687366041319368\\
55	0.687659673015179\\
56	0.688241153365799\\
57	0.689117442416254\\
58	0.689094247543209\\
59	0.688840540845209\\
60	0.689309835484116\\
61	0.69077921519867\\
62	0.692296308239198\\
63	0.690607969717305\\
64	0.687417089065763\\
65	0.684505388593389\\
66	0.681201003733499\\
67	0.679539317027983\\
68	0.679943587644424\\
69	0.68126889607081\\
70	0.682970937018548\\
71	0.683399370719794\\
72	0.68337716362255\\
73	0.682767969995914\\
74	0.681935987143201\\
75	0.681557469410172\\
76	0.681654088230165\\
77	0.683104129085339\\
78	0.685781054602103\\
79	0.688161751733229\\
80	0.689463180213991\\
81	0.690386581699466\\
82	0.692314916915624\\
83	0.697156423854616\\
84	0.702416632717911\\
85	0.703582566094149\\
86	0.701767987756783\\
87	0.698240393013788\\
88	0.694920301495758\\
89	0.693876223892146\\
90	0.693873708889302\\
91	0.693655524050992\\
92	0.691763521040824\\
93	0.688649258429357\\
94	0.686217408843408\\
95	0.685305120241564\\
96	0.684035067330134\\
97	0.682401605702688\\
98	0.682721069057237\\
99	0.683777991212358\\
100	0.684423822257973\\
101	0.685372328638147\\
102	0.686647649661052\\
103	0.687955561821304\\
104	0.687937760594647\\
105	0.687136349966859\\
106	0.687714669428776\\
107	0.689571635485443\\
108	0.690820200762096\\
109	0.691844589298435\\
110	0.69406271756582\\
111	0.697865582907153\\
112	0.70044580282545\\
113	0.70081932607453\\
114	0.700409042545388\\
115	0.700791511155703\\
116	0.702539184877944\\
117	0.703369559925115\\
118	0.703136303855229\\
119	0.702091371611984\\
120	0.699749813339278\\
121	0.696721168751155\\
122	0.694365360574852\\
123	0.693882119127358\\
124	0.693908564477027\\
125	0.692993684199865\\
126	0.690675221290497\\
127	0.688120422016162\\
128	0.687361181141926\\
129	0.688547586697702\\
130	0.689858513070452\\
131	0.690127642972602\\
132	0.688506273832356\\
133	0.685903542851147\\
134	0.684857314185073\\
135	0.684451950784722\\
136	0.684956707032289\\
137	0.685794879758436\\
138	0.68592320767302\\
139	0.68728160104011\\
140	0.688059361486745\\
141	0.687874991695113\\
142	0.687673108945986\\
143	0.686576423241492\\
144	0.68617887635922\\
145	0.68711478368735\\
146	0.689924400073869\\
147	0.694978275631866\\
148	0.697856091658909\\
149	0.699351172955049\\
150	0.699286784543512\\
};
\addlegendentry{$\varepsilon$-greedy}

\addplot [color=blue, solid, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0319143350540912\\
2	0.224339730980844\\
3	0.378908469904506\\
4	0.496414306678626\\
5	0.57215258205231\\
6	0.63324504650182\\
7	0.683545479720997\\
8	0.724173154148467\\
9	0.755291162935192\\
10	0.780250195002039\\
11	0.801391882359168\\
12	0.819794307218241\\
13	0.835685553943269\\
14	0.849144979433109\\
15	0.861717363771523\\
16	0.873444053358213\\
17	0.884171837900406\\
18	0.894273378560256\\
19	0.903456742684622\\
20	0.911797982127322\\
21	0.91948268341834\\
22	0.926512141848658\\
23	0.932944837863517\\
24	0.938687407171296\\
25	0.943882079331173\\
26	0.948683373543918\\
27	0.952993709354413\\
28	0.956802243362701\\
29	0.9603251720019\\
30	0.963640837770495\\
31	0.966795727227091\\
32	0.969540743390768\\
33	0.971886115076529\\
34	0.973974778690258\\
35	0.975872408453218\\
36	0.977780571165935\\
37	0.979443983093289\\
38	0.980955958179317\\
39	0.982588083641365\\
40	0.984092250497017\\
41	0.98545977997218\\
42	0.986659042656739\\
43	0.987797745099769\\
44	0.988948267403728\\
45	0.989919214881571\\
46	0.990833419674793\\
47	0.991838143427748\\
48	0.992758154352154\\
49	0.993442867180703\\
50	0.993873533785355\\
51	0.994297246929859\\
52	0.994830619414788\\
53	0.995317920668827\\
54	0.995739888620539\\
55	0.996153987496503\\
56	0.996524044551784\\
57	0.996816069558778\\
58	0.997024044551784\\
59	0.997136292317699\\
60	0.997233313757535\\
61	0.997372810125422\\
62	0.9975748279981\\
63	0.997848991063661\\
64	0.998121291481643\\
65	0.99834264169068\\
66	0.998487752234085\\
67	0.998558260269412\\
68	0.99863561584763\\
69	0.998760111379461\\
70	0.998939663130516\\
71	0.999100676470069\\
72	0.99919932352993\\
73	0.999224946511877\\
74	0.999214942108663\\
75	0.999220899228991\\
76	0.99923921215047\\
77	0.999288428704154\\
78	0.999341965220611\\
79	0.999369831565258\\
80	0.999400225490023\\
81	0.999394101607065\\
82	0.999405447412888\\
83	0.999454663966572\\
84	0.999497472419882\\
85	0.999560336869484\\
86	0.999641739730588\\
87	0.999733990227605\\
88	0.999812247765915\\
89	0.999806123882957\\
90	0.9997637076823\\
91	0.99976011137946\\
92	0.999799774509977\\
93	0.999875955448215\\
94	0.999894778077135\\
95	0.999845110543404\\
96	0.999820673738968\\
97	0.99983921215047\\
98	0.999888654194177\\
99	0.999911796785869\\
100	0.999894101607065\\
101	0.999899774509977\\
102	0.999930168434742\\
103	0.999969831565258\\
104	1.00000022549002\\
105	1.00000589839293\\
106	1\\
107	1\\
108	1\\
109	1\\
110	1\\
111	1\\
112	1\\
113	1\\
114	1\\
115	1\\
116	1\\
117	1\\
118	1\\
119	1\\
120	1\\
121	1\\
122	1.00000589839293\\
123	0.999994327097088\\
124	0.999975504468169\\
125	0.999954663966572\\
126	0.99993921215047\\
127	0.999954663966572\\
128	0.999975504468169\\
129	0.999994327097088\\
130	1.00001179678587\\
131	0.999994327097088\\
132	0.999969606075235\\
133	0.999960336869483\\
134	0.999969606075235\\
135	0.999994327097088\\
136	1.00000589839293\\
137	1\\
138	1\\
139	1\\
140	1\\
141	1\\
142	1\\
143	1\\
144	1\\
145	1\\
146	1\\
147	1\\
148	1\\
149	1\\
150	1\\
};
\addlegendentry{quasi $\varepsilon$-greedy}

\addplot [color=olive, solid, line width=2.0pt]
  table[row sep=crcr]{%
1	0.0332482749966623\\
2	0.223311064628817\\
3	0.376441722272929\\
4	0.493465482323137\\
5	0.56970182060282\\
6	0.631656631453174\\
7	0.682299907738251\\
8	0.722534405555317\\
9	0.753774293097622\\
10	0.778674280520348\\
11	0.799776538578301\\
12	0.818383380845491\\
13	0.834568137798287\\
14	0.848871029280297\\
15	0.861558460566397\\
16	0.87319246444951\\
17	0.883962377817221\\
18	0.893113650013896\\
19	0.90090101941488\\
20	0.907829029447096\\
21	0.914598705787255\\
22	0.921207251333073\\
23	0.927350001058989\\
24	0.933128030989298\\
25	0.938366402025048\\
26	0.943079053581145\\
27	0.947127474091995\\
28	0.950619938541504\\
29	0.95407466123547\\
30	0.957575504468169\\
31	0.961068431435256\\
32	0.964660609549371\\
33	0.968280785118428\\
34	0.97169899212265\\
35	0.974467766502716\\
36	0.976477296850824\\
37	0.978230950822068\\
38	0.980020840501597\\
39	0.981897697909905\\
40	0.983675788685586\\
41	0.985176122210845\\
42	0.986527699582018\\
43	0.987698872549884\\
44	0.988740565090608\\
45	0.989747412633499\\
46	0.990648765573638\\
47	0.991443484923379\\
48	0.992208200483029\\
49	0.992977806558264\\
50	0.993803145322793\\
51	0.994555791416688\\
52	0.995066627515071\\
53	0.995415226326079\\
54	0.995657132819296\\
55	0.9959\\
56	0.996154663966572\\
57	0.996420615011574\\
58	0.996715677306125\\
59	0.996954605239178\\
60	0.997179159498403\\
61	0.997417018708734\\
62	0.997688428704154\\
63	0.99798185384115\\
64	0.998224044551784\\
65	0.998382304821196\\
66	0.998445787013474\\
67	0.998454438476549\\
68	0.998504996432842\\
69	0.998654663966572\\
70	0.998803821792863\\
71	0.998906123882958\\
72	0.998978032048287\\
73	0.999033764737582\\
74	0.999100225490023\\
75	0.999136066827676\\
76	0.999175504468169\\
77	0.999218822628919\\
78	0.999245110543404\\
79	0.999290730794249\\
80	0.999345336033427\\
81	0.999394552587111\\
82	0.999411796785869\\
83	0.999388203214131\\
84	0.999399549019954\\
85	0.999448540083615\\
86	0.99953921215047\\
87	0.99966078784953\\
88	0.999751459916385\\
89	0.999806349372981\\
90	0.999800225490023\\
91	0.999769380585212\\
92	0.999784606911291\\
93	0.99983921215047\\
94	0.999924721021853\\
95	0.999981628351127\\
96	1.00000022549002\\
97	1.00000589839293\\
98	1.00000589839293\\
99	0.999994327097088\\
100	0.999969606075235\\
101	0.999960336869483\\
102	0.999969606075235\\
103	0.999994327097088\\
104	1.00000589839293\\
105	1\\
106	1\\
107	1\\
108	1.00000589839293\\
109	0.999994327097088\\
110	0.999969606075235\\
111	0.999966235262418\\
112	0.999975729958192\\
113	0.999958485759435\\
114	0.999899774509977\\
115	0.999859885889438\\
116	0.999893876117042\\
117	0.999970057055281\\
118	1.00000045098005\\
119	0.999975504468169\\
120	0.999960336869483\\
121	0.999969606075235\\
122	0.999994327097088\\
123	1.00001179678587\\
124	0.999994327097088\\
125	0.999975504468169\\
126	0.999954663966572\\
127	0.99993921215047\\
128	0.999954663966572\\
129	0.999981402861104\\
130	0.999988654194177\\
131	0.999981402861104\\
132	0.999954663966572\\
133	0.999945110543404\\
134	0.999948991063661\\
135	0.999945110543404\\
136	0.999954663966572\\
137	0.999975504468169\\
138	0.999994327097088\\
139	1.00000589839293\\
140	1.00000589839293\\
141	1.00000022549002\\
142	0.999963933172323\\
143	0.999935841337653\\
144	0.999924270041807\\
145	0.999933539247558\\
146	0.999960562359507\\
147	0.999984282574259\\
148	0.99998402880344\\
149	0.999964851855435\\
150	0.999925508016953\\
};
\addlegendentry{quasi $\varepsilon$-greedy with target recovery}

\end{axis}
\end{tikzpicture}

==> figures/AlgorithmDescription/varying_alpha/VaryingAlpha_alpha.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[%
width=75mm,
height=22mm,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=100,
xlabel style={font=\color{white!15!black}},
xlabel={Discrete time $k$},
ymin=0.2,
ymax=0.6,
ylabel style={font=\color{white!15!black}},
ylabel={$\alpha_k$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.61350944597318\\
2	0.601514630148689\\
3	0.589760361135498\\
4	0.578249164121914\\
5	0.566982322662146\\
6	0.555960104407064\\
7	0.545182102149288\\
8	0.534647414372707\\
9	0.524354744350204\\
10	0.514302455058208\\
11	0.504488614230044\\
12	0.494911046581695\\
13	0.48556749148466\\
14	0.476455875417512\\
15	0.467574858320134\\
16	0.458924813569979\\
17	0.450509690102775\\
18	0.442340993062786\\
19	0.434446902264338\\
20	0.426889321810805\\
21	0.419741489615446\\
22	0.412813016407869\\
23	0.406082524833914\\
24	0.399544274177132\\
25	0.393201674153008\\
26	0.387059356398923\\
27	0.381121803667884\\
28	0.375392827296209\\
29	0.369874973225361\\
30	0.364569607029866\\
31	0.359477555816136\\
32	0.354598659999378\\
33	0.349930027486165\\
34	0.345465366175786\\
35	0.341195242266547\\
36	0.337109452835042\\
37	0.333197491042661\\
38	0.329447526493577\\
39	0.325848082497863\\
40	0.322390753540911\\
41	0.31906888337647\\
42	0.315876938516334\\
43	0.312809672593241\\
44	0.309860967533515\\
45	0.307026300558615\\
46	0.304302152054294\\
47	0.301684951953595\\
48	0.299170954077577\\
49	0.296757964565761\\
50	0.294444152786164\\
51	0.29222905962833\\
52	0.290113666413198\\
53	0.288100345698588\\
54	0.286192640158606\\
55	0.284395540477759\\
56	0.282712134084834\\
57	0.2811423812504\\
58	0.27968273900885\\
59	0.278326182545756\\
60	0.27706116226265\\
61	0.275874606394713\\
62	0.274755326447056\\
63	0.273695921813013\\
64	0.272690694238487\\
65	0.271735525374319\\
66	0.27082763147049\\
67	0.269966642005225\\
68	0.269155346613563\\
69	0.268397223945687\\
70	0.267694795738462\\
71	0.267046822514458\\
72	0.266450165990244\\
73	0.265901064319079\\
74	0.265396128720706\\
75	0.264931251716208\\
76	0.264502908949315\\
77	0.264110105108325\\
78	0.263753008853527\\
79	0.263431162875329\\
80	0.263143448151725\\
81	0.262906785084771\\
82	0.262672190692211\\
83	0.262429529866198\\
84	0.262183697164274\\
85	0.261939870738207\\
86	0.261701245244205\\
87	0.261469614303798\\
88	0.261245972384881\\
89	0.261030780980649\\
90	0.260824142534823\\
91	0.260625880119897\\
92	0.26043561441806\\
93	0.260252851538076\\
94	0.260077040488662\\
95	0.259907583690991\\
96	0.259743857758004\\
97	0.259585233885776\\
98	0.25943110234148\\
99	0.259280905298491\\
100	0.259134164054275\\
};
\end{axis}
\end{tikzpicture}%

==> figures/AlgorithmDescription/varying_epsilon/VaryingEpsilon_epsilon.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}
\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[%
width=75mm,
height=22mm,
at={(0\textwidth,0\textwidth)},
scale only axis,
xmin=1,
xmax=300,
xlabel style={font=\color{white!15!black}},
xlabel={Discrete time $k$},
ymin=0.1,
ymax=0.8,
ylabel style={font=\color{white!15!black}},
ylabel={$\varepsilon_k$},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids
]
\addplot [color=red, line width=2.0pt, forget plot]
  table[row sep=crcr]{%
1	0.805601959585607\\
2	0.801276812501015\\
3	0.796658751058023\\
4	0.791753296224238\\
5	0.786564938639459\\
6	0.781097254383478\\
7	0.775352969317279\\
8	0.76933389002754\\
9	0.763040715409012\\
10	0.756472737682985\\
11	0.749627342350587\\
12	0.742499278062904\\
13	0.735079695044742\\
14	0.727356025912453\\
15	0.71932576492968\\
16	0.711084717398743\\
17	0.702701529574017\\
18	0.69416850411281\\
19	0.685505754120953\\
20	0.676731779164872\\
21	0.667861207325867\\
22	0.658911637803841\\
23	0.649904749048327\\
24	0.640861792427547\\
25	0.631801424541058\\
26	0.622740992306345\\
27	0.613697231461793\\
28	0.604684177694007\\
29	0.595710976818219\\
30	0.586786076144183\\
31	0.577917282179149\\
32	0.569112620430209\\
33	0.560382125138196\\
34	0.55174136477723\\
35	0.543211605504164\\
36	0.53481261473938\\
37	0.526554216123235\\
38	0.518439765835292\\
39	0.510469536697097\\
40	0.502644244056622\\
41	0.494967951115208\\
42	0.487443591926386\\
43	0.48007186676282\\
44	0.472847895423719\\
45	0.465759942231572\\
46	0.458792258240013\\
47	0.451923395510199\\
48	0.445135871020279\\
49	0.438424406350751\\
50	0.431794905964373\\
51	0.425256479311076\\
52	0.418818303651725\\
53	0.412489413172129\\
54	0.406281291413241\\
55	0.400208957055287\\
56	0.394286208787871\\
57	0.388522814431362\\
58	0.382925411670714\\
59	0.377497165654035\\
60	0.372236335289729\\
61	0.367137683650834\\
62	0.362192356278532\\
63	0.357387512857008\\
64	0.352703725736812\\
65	0.348114199023804\\
66	0.343592598499852\\
67	0.339115907962389\\
68	0.334667415992052\\
69	0.330239883010347\\
70	0.325837107963738\\
71	0.321472387510689\\
72	0.317157748482474\\
73	0.312902564299652\\
74	0.308716819800845\\
75	0.304609479662173\\
76	0.300588367855123\\
77	0.296655611324529\\
78	0.292807189318314\\
79	0.28903858561286\\
80	0.285350561951687\\
81	0.28175159860704\\
82	0.278257868280353\\
83	0.274886811135842\\
84	0.271648893318506\\
85	0.268544907582748\\
86	0.265569278842483\\
87	0.262713520219078\\
88	0.259964602832051\\
89	0.257308115407635\\
90	0.254734519270548\\
91	0.25224269975936\\
92	0.249834606793622\\
93	0.247509687645002\\
94	0.245260415526932\\
95	0.243067502134275\\
96	0.240906813448018\\
97	0.238755973415409\\
98	0.236601450885565\\
99	0.234439575762886\\
100	0.23227708867975\\
101	0.230133311117203\\
102	0.228034486215858\\
103	0.226008605883996\\
104	0.224074860692582\\
105	0.222237635574032\\
106	0.220488723159203\\
107	0.218816254041267\\
108	0.217210570570033\\
109	0.215668185559808\\
110	0.21418847787553\\
111	0.212767801272797\\
112	0.211398272938563\\
113	0.210069416848706\\
114	0.208766369893962\\
115	0.207467640897888\\
116	0.206149207907514\\
117	0.204793689375933\\
118	0.203397549501986\\
119	0.201971251230517\\
120	0.200531528979125\\
121	0.19909429187773\\
122	0.197671293376703\\
123	0.196269864375192\\
124	0.194895865008256\\
125	0.193553255433433\\
126	0.192244659658824\\
127	0.190971129810394\\
128	0.189736712970105\\
129	0.188552189407532\\
130	0.187430417793875\\
131	0.186384297952542\\
132	0.185417021206734\\
133	0.184517114113491\\
134	0.183667698025192\\
135	0.182853894933054\\
136	0.182064719165131\\
137	0.18129582185995\\
138	0.180548433666907\\
139	0.179824646686147\\
140	0.179123648145402\\
141	0.178441625191429\\
142	0.177771773535399\\
143	0.177107282952999\\
144	0.176445264464265\\
145	0.175788244862158\\
146	0.175140984046879\\
147	0.174511250114432\\
148	0.173908810585267\\
149	0.173342813955034\\
150	0.172819980934966\\
151	0.17233915289099\\
152	0.171890460871486\\
153	0.171458323979456\\
154	0.171026440872892\\
155	0.170580032247396\\
156	0.170109696025011\\
157	0.169615003476948\\
158	0.169104044259435\\
159	0.168586024027363\\
160	0.168062943918296\\
161	0.167531336703872\\
162	0.166989930318698\\
163	0.166439166452985\\
164	0.165883582342268\\
165	0.165334024520664\\
166	0.1648015220646\\
167	0.16429507564596\\
168	0.163820202799892\\
169	0.163378664701278\\
170	0.162968919484644\\
171	0.162584784548729\\
172	0.162217795813134\\
173	0.161864846555066\\
174	0.161527148442544\\
175	0.161206564099307\\
176	0.160903189003413\\
177	0.16061444785539\\
178	0.160338639040577\\
179	0.1600761118938\\
180	0.159829876102019\\
181	0.159604724821476\\
182	0.159405199346432\\
183	0.159236250407795\\
184	0.159105994252285\\
185	0.159024179685018\\
186	0.158998139146538\\
187	0.159027946281308\\
188	0.159106287461659\\
189	0.159220799782169\\
190	0.159357464956024\\
191	0.159502285428581\\
192	0.159640969771956\\
193	0.159763854218567\\
194	0.159868732640996\\
195	0.15996084315573\\
196	0.16004258041657\\
197	0.160107283316555\\
198	0.160144155306278\\
199	0.1601448355346\\
200	0.16010956589405\\
201	0.160046139877448\\
202	0.159963097036485\\
203	0.15986605807833\\
204	0.159758427737375\\
205	0.159644453986099\\
206	0.159529568390296\\
207	0.159418123951908\\
208	0.159308506904987\\
209	0.159195436431282\\
210	0.159071458153348\\
211	0.158929084896492\\
212	0.158764328909524\\
213	0.15857889926505\\
214	0.158378425819717\\
215	0.158167553498477\\
216	0.157945127062818\\
217	0.157706080013362\\
218	0.157445100465172\\
219	0.157157691287443\\
220	0.156842740546626\\
221	0.156506943810916\\
222	0.156162313288788\\
223	0.155820345371866\\
224	0.155487770990414\\
225	0.155170206017418\\
226	0.154875983915394\\
227	0.154613414305169\\
228	0.154386326044348\\
229	0.154192148350307\\
230	0.154022626051665\\
231	0.15386805080601\\
232	0.153718366163028\\
233	0.153563604841348\\
234	0.153398325869758\\
235	0.153222925496488\\
236	0.153040414656773\\
237	0.152856104788352\\
238	0.152674188059962\\
239	0.15249722374728\\
240	0.152328775048482\\
241	0.152175768384612\\
242	0.152045193260161\\
243	0.151939894930081\\
244	0.151859781083282\\
245	0.151805917723262\\
246	0.15177976444435\\
247	0.151783726181799\\
248	0.151820163205506\\
249	0.151885728500445\\
250	0.151972404197563\\
251	0.152074552318572\\
252	0.15218942359916\\
253	0.1523152308896\\
254	0.152448811856919\\
255	0.152583670467079\\
256	0.15271125722661\\
257	0.152822622390552\\
258	0.15290892223895\\
259	0.152963823407889\\
260	0.152983574902005\\
261	0.152968096715544\\
262	0.152924032532673\\
263	0.152857492058307\\
264	0.15277215039139\\
265	0.152671812420767\\
266	0.152559238290916\\
267	0.152435579969902\\
268	0.152298384104243\\
269	0.152146111604538\\
270	0.151981227760225\\
271	0.151810096564754\\
272	0.151643465561188\\
273	0.151492877940551\\
274	0.151363832461195\\
275	0.151255873540658\\
276	0.151163651315203\\
277	0.151076532986223\\
278	0.150985471790231\\
279	0.150885953369998\\
280	0.150777154404499\\
281	0.150662629958146\\
282	0.150548730006054\\
283	0.150442675811012\\
284	0.15035185842853\\
285	0.150280014935161\\
286	0.150218115627386\\
287	0.150191450060257\\
288	0.150189950169856\\
289	0.150208024474414\\
290	0.15024390681369\\
291	0.150297600270468\\
292	0.150369760909813\\
293	0.150461236755461\\
294	0.150572800984955\\
295	0.150705063654517\\
296	0.150858508715183\\
297	0.151033464464073\\
298	0.151230092966172\\
299	0.151448459317859\\
300	0.151688587312106\\
};
\end{axis}
\end{tikzpicture}%
